Fresh Caching of Dynamic Contents using Restless Multi-armed Bandits

We consider a dynamic content caching problem wherein the contents get updated at a central server, and local copies of a subset of contents are cached at a local cache associated with a Base station (BS). When a content request arrives, based on whether the content is in the local cache, the BS can decide whether to fetch the content from the central server or serve the cached version from the local cache. Fetching a content incurs a fixed fetching cost, and serving the cached version incurs an ageing cost proportional to the age-of-version (AoV) of the content. The BS has only partial information regarding AoVs of the contents. We formulate an optimal content fetching and caching problem to minimize the average cost subject to cache capacity constraints. The problem suffers from the curse of dimensionality and is provably hard to solve. We formulate this problem as a continuous time restless multi-armed bandit process (RMAB), where a single content problem of the corresponding RMAB is a partially observable Markov decision process. We reformulate the single content problem as a semi-Markov decision process, prove indexability, and provide a Whittle index based solution to this problem. Finally, we compare the performance with recent work and show that our proposed policy is optimal via simulations.

==> proof_of_monotonicity.tex <==
The proof of $(a)$, we make use of the value iteration algorithm.
\begin{align}
    V_{i+1}(\tau)=\min\{c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}V_i(t+\tau)dt, \, c_f-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}V_{i}(t)dt\}
\end{align}
Since, value iteration algorithm converges to the value function~\cite{puterman2014markov}, it is sufficient to show that for $\tau_1\leq \tau_2$, 
\begin{align}
    V_i(\tau_1)\leq V_i(\tau_2) \forall\,\, i\in \mathbb{Z}_{+} \label{ineq: value_iteration}
\end{align}
To prove this, we follow induction method. We define: $V_0(\tau)=0\,\forall \,\tau \geq 0$. Hence, ~\eqref{ineq: value_iteration} is satisfied for $i=0$. We assume, $V_n(\tau_1)\leq V_n(\tau_2)$ and we prove that,  $V_{n+1}(\tau_1)\leq V_{n+1}(\tau_2)$.  We note that, $Q(\tau_1,0)=c_a \lambda \tau_1-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}V_i(t+\tau_2)dt \leq Q(\tau_2,0)=c_a \lambda \tau_1-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}V_i(t+\tau_2)dt$. We further note that,  $Q(\tau,1)$ is constant.Hence, $V_{n+1}(\tau_1)\leq V_{n+1}(\tau_2)$. \\
To prove part~$(b)$, we make use of the following facts:\begin{enumerate}
    \item   $Q(\tau,0)$ is non-decreasing in $\tau$ as $h(\tau)$ is non-decreasing in $\tau$.
    \item $Q(\tau,1)$ is constant.
\end{enumerate} Hence, there exists a $\tau^{\ast}$ such that the following holds:\begin{align*}
h(\tau)=\begin{cases} c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t+\tau)dt &\,\,\forall \tau \leq\tau^*\\
h, &\,\,\forall \tau \geq \tau^*
\end{cases}  
\end{align*}
At $\tau=\tau*$, $h(\tau^*)=h\implies  c_a \lambda \tau^{\ast}-\frac{\theta}{\beta}+h=h\,\implies \theta=\beta c_a \lambda \tau^\ast$
For $\tau<\tau^\ast$,
\begin{align}
   h(\tau) = &c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t+\tau)dt \nonumber \\
   = &c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\tau^\ast-\tau}\beta e^{-\beta t}h(t+\tau)dt +\int_{\tau^\ast-\tau}^{\infty}\beta e^{-\beta t}h(t+\tau)dt \label{diff_equ_firstproblem}
\end{align}
Solving the differential equation~\eqref{diff_equ_firstproblem}, we get\begin{align}
  h(\tau)=c_a \lambda \tau +\beta c_a \lambda(\tau \tau^\ast-\frac{\tau^2}{2})+C_1 \label{sol_to_diff_equ_firstproblem} 
\end{align} where $C_1$ is an integration constant. We note that, $h(\tau^\ast)=h$ and $h(0)=h-c_f$. Hence, $C_1=h-c_f$. Hence we obtain,
\begin{align*}
h(\tau)=\begin{cases} c_a \lambda \tau +\beta c_a \lambda(\tau \tau^\ast-\frac{\tau^2}{2})+ h-c_f &\,\,\forall \tau \leq \tau^*\\
h, &\,\,\forall \tau > \tau^*
\end{cases}  
\end{align*}
\[h= c_a\lambda\tau^\ast+\beta c_a \lambda\frac{\tau^{\ast2}}{2}+h-c_f\]
\[\implies \tau^{\ast2}+\frac{2}{\beta}\tau^\ast-\frac{2c_f}{\beta c_a \lambda}=0 \]
\[\implies \tau^\ast=-\frac{1}{\beta}+\sqrt{\frac{1}{\beta^2}+\frac{2c_f}{\beta c_a \lambda}}=\frac{1}{\beta}\left(\sqrt{1+\frac{2c_f\beta}{c_a \lambda}}-1\right)\]
The optimal cost, $\theta=c_a\lambda \left(\sqrt{1+\frac{2c_f\beta}{c_a \lambda}}-1\right)$


==> single_content_with_infinite_cache.tex <==
\subsection{Single content with infinite caching capacity:}
Let us assume that $\lambda$ and $\beta$ are the rate at which the content gets updated at the server and the request arrives at the BS, respectively. We note that action is either serving the stale version or fetching the fresh content from the cloud when a request for content arrives. We define the state at $t$ as the time since fresh content is fetched. We define $a(t)$ as the action at time $t$. When a request arrives, the following actions are possible: $a(t)=\begin{cases}
    1,\,\, \text{ fetch a fresh content} \\
    0, \,\, \text{ serve the stale version}
\end{cases}$.\\
If there are no requests at time $t$, $a(t)=0$. Let $\tau$ be the state at time $t$. Hence, $\tau=t-\max\{l < t : a(l)=1\}$. Let $\theta$ be the optimal average cost. Let $Q(\tau,a)$ be the action-value function. 
\begin{align}
    Q(\tau,1)& =  c_f-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t)dt \\
     Q(\tau,0)& =  c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t+\tau)dt
\end{align}Then, the Bellman equations are given by,
\begin{align*}
    h(\tau)=\min \left \{ c_f-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t)dt, c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t+\tau)dt\right \}
\end{align*}
where $h(\tau)$ and $\theta$ are relative cost for state $\tau$ and
average optimal cost. 
\begin{theorem} \label{thm:1}
\begin{enumerate} [(a)]
    \item $h(\tau)$ is non-deceasing in $\tau$ for $\tau \geq 0$.\label{statement:monotonicity}
%    \item $h$ is not unique but $h(\tau_1)-h(\tau_2)$ is unique  $\forall \,\, \tau_1,\tau_2 \geq 0$
    \item The optimal policy is of threshold type, i.e., $\exists$ a $\tau^{*}$ s.t. $ c_a \lambda \tau-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t+\tau}h(t+\tau)dt > c_f-\frac{\theta}{\beta}+\int_{0}^{\infty}\beta e^{-\beta t}h(t)dt$ $\forall$ $\tau>\taustar$ and $\tau ^{\ast}=-\frac{1}{\beta}+\sqrt{\frac{1}{\beta^2}+\frac{2c_f}{\beta c_a \lambda}}$
\end{enumerate}
\end{theorem}
\begin{proof}
The proof can be found in Appendix~\ref{appendix:proof_theorem_1}. 
\end{proof}
If we replace $\beta$ with $\beta p_n $
 and $\lambda$ with ${\lambda}_n$, we get the threshold $\tau_n^{\ast}$ for each content $n$. Hence, $\tau_n^{\ast}=\frac{1}{\beta p_n}\left(\sqrt{1+\frac{2c_f\beta p_n}{c_a \lambda_n}}-1\right)$. Furthermore, the optimal cost is $\sum_n \theta_n=\sum_nc_a\lambda_n \left(\sqrt{1+\frac{2c_f\beta p_n}{c_a \lambda_n}}-1\right)$%{\it Myopic Policy:}
%Let $\tau^0$ be the time after which the action will be to fetch the content always under myopic policy. Hence, $\tau^0=\frac{c_f}{c_a \lambda}$. Hence, the average cost under myopic policy is $\theta'=\int_{0}^{\tau^0}c_a\lambda t \beta e^{-\beta t}dt+\int_{\tau^0}^{\infty}c_f\beta e^{-\beta t}dt$
